Treatment Effect Detection with Controlled FDR under Dependence for Large-Scale Experiments

Online controlled experiments (also known as A/B Testing) have been viewed as a golden standard for large data-driven companies since the last few decades. The most common A/B testing framework adopted by many companies use "average treatment effect" (ATE) as statistics. However, it remains a difficult problem for companies to improve the power of detecting ATE while controlling "false discovery rate" (FDR) at a predetermined level. One of the most popular FDR-control algorithms is BH method, but BH method is only known to control FDR under restrictive positive dependence assumptions with a conservative bound. In this paper, we propose statistical methods that can systematically and accurately identify ATE, and demonstrate how they can work robustly with controlled low FDR but a higher power using both simulation and real-world experimentation data. Moreover, we discuss the scalability problem in detail and offer comparison of our paradigm to other more recent FDR control methods, e.g., knockoff, AdaPT procedure, etc.

==> four_procedure_comparisons.tex <==



==> outline.tex <==
Title:
Adaptive False Discovery Rate Control under Dependence for Large-Scale Online Controlled Experiments

** Main contribution of this paper:
1) Establish ATE detection problem as FDR control problem

2) Demonstrate how adaptive BH method improve power based on simulation and real-world empirical data with baseline of traditional BH method.

3) Compare the adaptive BH method to another popular FDR control algorithm knock-off method.

** Some discussions that can be included:
the comparison with knock-off can include the following:
1. power 
2. computational cost/scalability
# maybe knockoff is better in high-dimensional case? but A/B testing is not high-dimensional

** Some questions to address:
1) Can we think of other applications other than the basic ATE detection? -- this can extend to heterogeneous treatment detection, and we can talk about them under discussion maybe

2) how to show scalability?

Abstract:

1. Introduction:
- why do we care about FDR control
    - if not, type I error will become to high

2. Preliminaries
2.1 The definition of metrics and ATE under Rubin Causal model
- see ref:https://alexdeng.github.io/public/files/wsdm2017-rup.pdf
 
2.2 naive approach and its caveat
- a simulation plot comparing when we do not consider the correlation matrix (see in Will's paper how they generate different correlation matrix for simulation)

3. Detection of ATE using adaptive FDR methods

3.1 dependence BH method
- steps 1. 2. 3., ...

3.2 simulation
- FDR vs signal size; power vs signal size in parallel

3.3 Empirical results
- run on real experiments,(find an experiment that has multiple groups and metrics) we can have a plot show treatment effect vs metrics, and mark significant metrics with different colors detected from different methods

4. Discussion
4.1 Comparison with knock-off method
- first, simulation based on both standard Gaussian distribution and real-experiment data
- then, compare with linkedin's result in the same setting (similar as figure 3).

4.2 Scalability

4.3 (Extension to Heterogeneous Treatment Effect Detection)

5. Literature Review

6. Conclusion and future work
